Can You See Me Now? A Measurement Study of Zoom, Webex, and Meet

Since the outbreak of the COVID-19 pandemic, videoconferencing has become the default mode of communication in our daily lives at homes, workplaces and schools, and it is likely to remain an important part of our lives in the post-pandemic world. Despite its significance, there has not been any systematic study characterizing the user-perceived performance of existing videoconferencing systems other than anecdotal reports. In this paper, we present a detailed measurement study that compares three major videoconferencing systems: Zoom, Webex and Google Meet. Our study is based on 48 hours' worth of more than 700 videoconferencing sessions, which were created with a mix of emulated videoconferencing clients deployed in the cloud, as well as real mobile devices running from a residential network. We find that the existing videoconferencing systems vary in terms of geographic scope, which in turns determines streaming lag experienced by users. We also observe that streaming rate can change under different conditions (e.g., number of users in a session, mobile device status, etc), which affects user-perceived streaming quality. Beyond these findings, our measurement methodology can enable reproducible benchmark analysis for any types of comparative or longitudinal study on available videoconferencing systems.

==> sections/07_conclusion.tex <==
%%%%%%%%%%%%%%%%%%%%%%
\section{Conclusion}
\label{sec:conclusion}
%%%%%%%%%%%%%%%%%%%%%%
TODO


==> sections/table.tex <==
\begin{table}[t]
\scriptsize
\centering
\setlength\tabcolsep{3pt}
\caption{Mean data rate and median CPU usage under variable videconference sizes (3/6/11 participants). Each cell reports statistics for S10/J3.}
\label{tab:comp}
\begin{tabular}{p{1cm} p{2cm} p{1.3cm} p{2cm} p{1.3cm}}
\toprule
      ~          & \begin{tabular}{@{}l@{}} \textbf{FullScreen}\\\textbf{Data Rate (Mbps)}\end{tabular} & \begin{tabular}{@{}l@{}} \textbf{}\\\textbf{CPU (\%)}\end{tabular} & \begin{tabular}{@{}l@{}} \textbf{Gallery}\\\textbf{Data Rate (Mbps)}\end{tabular}& \begin{tabular}{@{}l@{}} \textbf{}\\\textbf{CPU (\%)}\end{tabular}\\
\toprule
\multicolumn{5}{c}{\textbf{N=3}} \\
\midrule
    \textbf{Zoom}      & 0.85/0.9    & 164/186   & 0.33/0.37 & 102/148 \\
    \textbf{Webex}     & 1.76/0.9    & 148/183   & 0.57/0.59 & 149/186 \\
    \textbf{Meet}      & 2.08/2.13   & 205/190   & 2.08/2.11 & 209/200 \\
\midrule
\multicolumn{5}{c}{\textbf{N=6}} \\
\midrule
    \textbf{Zoom}      & 0.92/0.94   & 189/212   & 0.71/0.73  & 101/152  \\
    \textbf{Webex}     & 1.75/0.9    & 140/195   & 0.43/0.47  & 155/184  \\
    \textbf{Meet}      & 2.25/2.33   & 257/211   & 2.15/2.24  & 235/219  \\
\midrule
\multicolumn{5}{c}{\textbf{N=11}} \\
\midrule
    \textbf{Zoom}      & 0.91/0.96   & 191/211   & 0.73/0.75  & 100/150  \\
    \textbf{Webex}     & 1.76/0.89   & 141/194   & 0.48/0.43  & 154/182  \\
    \textbf{Meet}      & 2.24/2.36   & 258/210   & 2.16/2.26  & 236/220  \\
\bottomrule
\end{tabular}
\vspace{-0.2in}
\end{table}

%python3 paper-plotter.py logs/1621614939/log-script-1621614939 [for run with N VMs]

